Traveling Waves Encode the Recent Past and Enhance Sequence Learning

Traveling waves of neural activity have been observed throughout the brain at a diversity of regions and scales; however, their precise computational role is still debated. One physically inspired hypothesis suggests that the cortical sheet may act like a wave-propagating system capable of invertibly storing a short-term memory of sequential stimuli through induced waves traveling across the cortical surface, and indeed many experimental results from neuroscience correlate wave activity with memory tasks. To date, however, the computational implications of this idea have remained hypothetical due to the lack of a simple recurrent neural network architecture capable of exhibiting such waves. In this work, we introduce a model to fill this gap, which we denote the Wave-RNN (wRNN), and demonstrate how such an architecture indeed efficiently encodes the recent past through a suite of synthetic memory tasks where wRNNs learn faster and reach significantly lower error than wave-free counterparts. We further explore the implications of this memory storage system on more complex sequence modeling tasks such as sequential image classification and find that wave-based models not only again outperform comparable wave-free RNNs while using significantly fewer parameters, but additionally perform comparably to more complex gated architectures such as LSTMs and GRUs.

==> sections/experiments_waves.tex <==
\section{Experiments: On the Emergence of Wave-like dynamics}
Before we analyze the impact of biasing our networks towards wave-like activity, we first investigate how the hidden state dynamics are affected by different choices of recurrent connections, and verify that wave-like dynamics do indeed emerge. 

\textbf{Qualitative Analysis}
\label{sec:learning_waves}
In the following experiments we visualize the hidden state of our networks after training on a simple sequence modeling task described more thoroughly in the next section (sMNIST). By plotting the hidden state over the length of the sequence (time) it becomes visually clear which models posses wave-like dynamics. 

For example in Figure \ref{fig:waves}, we see that for both locally-connected $\mathbf{U}$ (left) and convolutional $\mathbf{U}$ (mid) models, waves are clearly visible in the hidden state by the end of training. Specifically, the only difference between these two moedls being that the locally-connected layer does not share paramerers over spatial locations. Such dynamics are reminiscent of prior work \cite{nwm} and noticeably more structured than the dynamics of fully connected RNNs (right). We see that locally connected RNNs exhibit traveling waves over shorter distances and in multiple directions simultaneously (owing to their diverse unshared local connectivity), while convolutional RNNs exhibit more global waves which all travel in the same direction (recipriocally owing to their shared connectivity over all locations).

\begin{figure}[h!]
\vspace{-0mm}
    \centering
    \includegraphics[width=0.9\textwidth]{figures/Waves_w_FC.png}
    \caption{Example of traveling waves in the hidden state $\mathbf{h}_t$ of a Locally-connected RNN (left) a convolutional RNN (mid), and a fully connected simple RNN (right) after training on a simple sequence modeling task. We see that despite none of the models having wave-like dynamics at initalization (not yet pictured, coming soon), models with local connectivity eventually learn to use traveling waves in order to solve their task.}
    \label{fig:waves}
\end{figure}

In Figure \ref{fig:2d_waves}, we depict the hidden state over time (top) and the estimated instantaneous phase \cite{Davis2021} (bottom), for an RNN with a 2-dimensional convolutional recurrent matrix $\mathbf{U}$ applied over a similarly 2-dimensional hidden state. We again see similar structure to prior work. In the remainder of this paper we stick with one-dimensional hidden states as they appear to be more memory efficient while still achieving the same benefits of traveling waves, and leave investigation of the further benefits of higher dimensional hidden states to future work.

\begin{figure}[h!]
\vspace{-0mm}
    \centering
    \includegraphics[width=0.8\textwidth]{figures/waves_2d_rnn.png}
    \caption{Example of 2-dimensional traveling waves in the (2D) hidden state $\mathbf{h}_t$ of a convolutional recurrent neural network. We see the waves are qualitatively similar to those of prior work \cite{nwm}.}
    \label{fig:2d_waves}
\end{figure}

\textbf{Quantitative Analysis}
In addition to the above qualitative analysis, we strive to compare diffent settings of our model quantiatively in terms of their abiliity to generate wave-like dynamics. To achieve this, we leverage methods recently developed in the computational neuroscience community \cite{Davis2021}, specifically those designed to compute the fraction of wave activity from neural recordings. 

\begin{itemize}
    \item Introduce metrics (define hilbert transform and instantaneous velocity / phase)
    \item Measure Percent Waves for Locally-connected RNN, Convolutional RNN and FC-RNN.
\end{itemize}

In the end we see that convolutional layers exhibit significantly more wave-like dynamics than their counterparts, supporting oour decision to use them in the remaining sections of this work.
